Federated Learning Over Images: Vertical Decompositions and Pre-Trained Backbones Are Difficult to Beat

We carefully evaluate a number of algorithms for learning in a federated environment, and test their utility for a variety of image classification tasks. We consider many issues that have not been adequately considered before: whether learning over data sets that do not have diverse sets of images affects the results; whether to use a pre-trained feature extraction "backbone"; how to evaluate learner performance (we argue that classification accuracy is not enough), among others. Overall, across a wide variety of settings, we find that vertically decomposing a neural network seems to give the best results, and outperforms more standard reconciliation-used methods.

==> experiments.tex <==
\section{Experiments}

\noindent \textbf{Setup.} 
We compare \textsc{Verdove} with various other state-of-the-art federated methods FedAvg \cite{fedavg}, FedProx \cite{fedprox}, FedAdam \cite{fedopt}, FedNova \cite{fednova}, and MOON \cite{moon}. Additionally, we compare with \textsc{VerdoveProx}, a hybrid method where we apply FedProx's proximal objective in \textsc{Verdove} local training. In addition, we have as an additional baseline the full backpropagation, i.e. without using a pretrained backbone, training with FedProx. 
We conduct experiments on a diverse and broad range of image classification datasets: (1) CUB-200-2011 \cite{birds}, (2) Aircraft \cite{aircraft}, (3) Stanford Cars \cite{cars}, (4) VGGFlowers \cite{flowers}, (5) VGGTextures \cite{dtextures}, and (6) CIFAR100 \cite{cifar}. The input images are passed through ResNet101\cite{resnet} and DenseNet121\cite{densenet} CNNs, pretrained on ImageNet \cite{imagenet}, to generate features which are concatenated. For all these experiments we use a single-hidden-layer multi-layer perceptron. The models have 1000 hidden nodes as the base global model architecture, except the VERDOVE methods where we scale the number of nodes based on the number of users in the training (3000 for 10 devices, 6000 for 20, 9000 for 30, 18000 for 60). In the VERDOVE methods case, this is to ensure the client models are not too small and we found that 300 hidden layers for the partitioned client models to work well in general. Although the central models are certainly overparamterized for the needs of these datasets, we demonstrate that we do not incur any computational or communication overhead and in fact show that VERDOVE performs better in these metrics. For the full backpropagation experiments, we use ResNet18 as the central model. 

Our main federated scenario consists of either $100$ or $1000$ clients and we consider cases of $10\%$ and $30\%$ randomized device participation for $100$ clients and $2\%$ and $6\%$ for $1000$ clients in each round. For \textsc{Verdove} and \textsc{VerdoveProx}, the hidden layer is divided by the number of participants in a given local round; however as stated in the previous paragraph we have normalized the local model size to $300$ hidden neurons.  

We implement \textsc{Verdove}, \textsc{VerdoveProx}, as well as the other methods in PyTorch \cite{pytorch}. For tuning our methods, we use the CUB-200-2011 dataset as our validation dataset. Additionally, we have separate sets of tuned hyperparameters for each case of client participation. In all cases, we use a learning rate of $0.01$ as we found this to give stable convergence in all algorithms except FedAdam.  
\textcolor{blue}{Ed: I'll need to rewrite this section as my method of choosing hyperparamters has slightly changed}
We consider the number of local iterations of mini-batched gradient descent as a hyperparameter with either 1, 5, or 25 iterations.  
For FedProx and \textsc{VerdoveProx} we have additional proximal hyperparameter ranging in 0.05, 0.1, 0.15, and 0.2; we have run \textsc{VerdoveProx} with 0.2 proximal term in all cases while FedProx with 0.05 in cases except the FLOP optimized 10\% usage case where we used 0.2. For MOON, we have parameters $\mu$, the coefficient of the contrastive term, and $\tau$, the temperature of the contrastive term; we have chosen $\mu=1, \tau=0.5$ for the FLOP minimizing case and $\mu=10, \tau=1$ for the communication minimizing case. As we emphasize that our parameters should be "out of the box", we use these same parameters for all datasets after tuning on CUBBirds-2011.

We simulate non-i.i.d. data with a Dirichlet distribution, a standard method in federated learning \cite{measuring_noniid, moon, fed_noniid}. Given Dirichlet parameter $\alpha$ and for each dataset we have class $i$ and client $j$, we sample $r_{i,j}\sim DIR(\alpha)$ as the proportion of client $j$'s data would be class $i$. Each client in total has 500 local image samples and we choose $\alpha=0.01$ to represent a very skewed data distribution. Additionally we test on the $\alpha=100$ (i.i.d.) scenario, but we opt to only consider the $10\%$ as identical client data distributions means different client participation rates will only 

Additionally, for the VGG Textures dataset we also compare with FedAvg and FedProx applied on a full backpropagation training ResNet34. In this case, our Dirichlet data distribution ranges in $\alpha\in [0.01, 1, 100]$, ranging from very skewed to i.i.d. These results are presented in \ref{fig:fullbackprop_res}

\subsection{Evaluation Metrics and Accuracy}

For each dataset, we determine the best final accuracy among all tested methods, presented in ~\cref{table:final_acc10}, ~\cref{table:final_acc30}, ~\cref{table:final_acc02}, and ~
\cref{table:final_acc06}. 
These final accuracies were determined over 1000 communication rounds for FedProx and MOON, 1000 rounds for FedAvg, and 4000 for \textsc{VERDOVE} and \textsc{VERDOVEProx}. 
The reason for the disparity in communication rounds is that different algorithms perform different amounts of computation for a single communication round and hence we note that communication rounds are misleading in the federated setting.  

Per dataset we take this best accuracy from these tables, and determine the smallest number of FLOPs to first reach 90\% of this best accuracy and likewise the smallest number of bytes communicated in each communication round to first reach 90\% of this accuracy. 
Our choice in this metric is intuitive: \textit{We want to fairly compare the FLOP and bytes transferred efficiency by controlling for some high accuracy.} 
These metrics also have a practical interpretation that, in this device constrained federated setting, we cannot feasibly train forever and must choose some reasonable point (such as the 90\% cutoff) to consider the model ``converged''. To smooth out the averages, we compute over a 10 point sliding window to avoid algorithms with spiky and inconsistent convergence curves (In particular FedAdam). 

We set a timeout at 100000 GFlops of total computation and 5000 GB of communicated data where if a method fails to reach the target accuracy within these timeout cutoffs we consider the algorithms to have failed in the task (Marked in the tables as "FAIL"). This timeout is particularly relevant for the full backpropagation FedProx baseline where the trained ResNet18 is drastically larger than the MLP we train for other methods. 

First, we note that in general the final accuracies in the i.i.d. cases are roughly the same and differ by at most 2\% in the case of CIFAR100. This is unsurprising as the theory in many of these algorithms \cite{fedavg, fedprox, fednova, ist, masked_neurons} is almost always done on the assumption of i.i.d. data distributions and are expected to perform well in both final accuracy and convergence rate in this scenario. We observe as well that FedProx and MOON perform better in the i.i.d. case than FedAvg by about 0.5-1\%, and that VERDOVE methods edge out even further, except in the case of CIFAR100 where FedAvg performs best. 

For all datasets except VGG Flowers and VGG Textures, FedAdam exhibits a significant accuracy gap. Additionally, we observe that FedAdam (\ref{figureTODO}) is very fast in converging to its peak in these cases but heavily drops off immediately afterwards. Combined with the observed instability in the non-i.i.d. case for FedAdam (\ref{figureTODO}), this consequently results in an uncertainty in where to stop training that makes FedAdam an impractical choice for the federated setting. This is noteworthy as although acceleration such as Adam is useful in centralized machine learning, in this federated setting it exhibits pathological behaviors that hurt its usefulness. 

More interesting however is the deviation from the i.i.d. scenario once we have very skew Dirichlet distributed data. The first key observation is that FedProx and MOON have degraded performance relative to FedAvg as they are now 2-3\% behind FedAvg in final peak accuracy. While VERDOVE methods achieve the highest final accuracies, we note that our experimental setup for these use a significantly (3-12x) larger central model size so we must emphasize that the final accuracy does not tell the full story in this case. 

Consistent with our results in \ref{fig:fedprox_full}, the full-backprop case fails on the non-i.i.d. experiments to reach the target accuracy for all datasets; for many datasets the full-backprop method does not even break 5\% accuracy. The full backpropagation method does exhibit higher accuracies for the VGG Flowers and VGG Textures datasets, but nevertheless the model is too large that it cannot converge to the same final accuracies within our set timeout. 

We also note that between 10 and 30\% participation experiments the final accuracies are generally similar and in a few cases, final accuracies decrease in the higher device case. This is also the case between 2 and 6\% scenarios suggesting that with sufficient communication rounds to sample enough device local data, greater fraction of user participation does not significantly change the final accuracies, which can be useful in real-world federated training where we assume client participation may be sparse and sporadic. In contrast, we note that between 100 versus 1000 total devices scenarios, the final accuracies jump significantly as the 1000 device final accuracies are near the same performance of the i.i.d. case, again suggesting that more overall users but sparser sampling of these users helps in general for federated algorithms.  

VERDOVEProx in general has slightly higher accuracy than VERDOVE except in a few cases. Additionally we note that outside of the i.i.d. case VERDOVE methods perform poorly on the CIFAR100 dataset, especially in the 1000 user scenario where the gap is as large as 10\%. A possible cause is that our local models of 300 hidden neurons are not large enough to capture the dataset. In terms of final accuracies, VERDOVE methods also perform comparable to FedProx and MOON in the lower participation case, but have the highest accuracies in the higher participation cases. We note that we use more local training in the higher participation cases and that local training helps with the Cars dataset. 

\subsection{Computation Efficiency}

\input{tables/flop_table_10.tex}

\input{tables/flop_table_30.tex}

\input{tables/flop_table_02.tex}

\input{tables/flop_table_06.tex}

\input{tables/flop_table_10_iid.tex}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Accuracy over Floating Point Operations (Birds dataset).pdf}
    \caption{\label{fig:birds_flops} Accuracy over floating point operations for the CUB-200-2011 dataset in the 30\% case. The dashed line represents the 90\% best accuracy threshold that we compare against. \textcolor{red}{Tasos: similarly to above. Remove title (per my taste), increase fontsize for axis, legends; make curves more thick.}}
\end{figure}

We use the FlopCountAnalysis tool in the Python \textit{fvcore} \cite{fvcore} package to estimate the number of floating point operations per stochastic gradient descent step in the model. In the case of MOON, we double this estimate as each step uses two additional forward propagations for computing the representations used in its local training. Per communication round, we multiply this estimate by the number of local SGD rounds and the number of participating client devices. As \textsc{Verdove} uses smaller local models, the estimated FLOP footprint of each local round for \textsc{Verdove} methods is smaller. \cref{table:flop10}, \cref{table:flop30}, \cref{table:flop02}, \cref{table:flop06}, and \cref{table:flop10iid} show the number of GFLOPs to reach 90\% of the top accuracy for each dataset for respective total client and client participation rate cases as well as i.i.d. versus non-i.i.d. We set a timeout of 100k GFlops and we fill in "FAIL" in these tables for timedout entries. 

In the i.i.d. case \ref{table:flop10iid} convergence to 90\% is expectedly fast. Moreover, due to the inherent model reduction in VERDOVE, it outperforms all other methods and except for Stanford Cars dataset the speed up is at least 3 times the fastest averaging algorithm (In Stanford Cars, both FedAvg and VERDOVE have similar GFLOPs). FedAdam and the full backpropagation FedProx both have poor performance even in the i.i.d. case, the former due to instability during convergence (\ref{figureTODO}) while the latter converges too slowly for the amount of FLOPs used. Comparing the non-i.i.d. to the i.i.d. cases the gap in GFLOP performance has at least 10x faster for i.i.d. but this gap is typically as much as 30x indicating the widely different problem settings and dificulty between i.i.d. and non-i.i.d. data.    

In the non-i.i.d. case, VERDOVE and VERDOVEProx generally outperforms other methods for the CUB-Birds, VGG Flowers, Aircraft, and VGG Textures datasets while in the remaining datasets Stanford Cars and CIFAR100 FedProx and MOON typically perform better, except in the case 30\%, 100 device case where these two methods "FAIL" and FedAvg is instead the fastest converging. FedNova appears to be consistently worse than FedAvg except in the case of the 1000 device cases of the Aircraft dataset. Neither FedAdam nor the full backpropagation FedProx can reach the 90\% threshold and are marked as FAIL, with the sole exception of FedAdam on 6\% participation VGG Flowers but even in this case it lags behind FedAvg and FedNova.  

Comparing FedAvg and FedProx, FedProx consistently has faster GFLOP convergence except in FAIL cases and in Stanford Cars (i.i.d.). The speedup ranges from 1.75 times (Stanford Cars, 2\%, 1000 devices) to as much as 30 times (Aircraft, 6\%, 1000 devices). Meanwhile, FedProx and MOON have approximately a 2x speed gap, which is consistent with the doubled overhead in MOON due to the extra forward passes although remarkably MOON is faster than FedProx in the VGGTextures case of 30\% on 100 devices. However, despite the consistent improvement over FedAvg by using a proximal term (Either directly or MOON's contrastive proximal loss), we do not see the same gains between VERDOVE and VERDOVEProx and we see similar GLOP counts for both algorithms. \cref{fig:birds_flops} highlights this speed at which vertical decomposition methods achieve our 90\% best accuracy threshold faster compared to other methods.  

In a few cases, e.g. FedProx on CUB-Birds with 2\% participation on 1000 devices versus 10\% on 100 devices, the GFLOP usage is lower for many methods despite the increased overall device participation (And hence per communication round GLOP usage). However, we do not see similar advantages between 10\% versus 30\% suggesting that increasing user count is the main cause of this phenomenon and again suggests high quantities of users helps with federated learning even if a smaller fraction of them participate in the training. 

An important caveat of FedProx and MOON is that for a large set of non-i.i.d. cases they fail to reach the 90\% best accuracy cutoff, specifically for the CUB-Birds and Stanford Cars datasets. However, despite FedAvg being more consistent its GFLOP performance can be one order of magnitude higher than FedProx/MOON and two orders of magnitude higher than VERDOVE. 

This indicates that while FedAvg can consistently achieve relatively high accuracy the trade off is that it also has a drastically worse computational overhead compared to alternatives. On the other hand, except for CIFAR100 in the non-i.i.d. cases, VERDOVE methods are also consistent at reaching the highest or second highest accuracies in contrast to FedProx/MOON, but without that extreme computation overhead that FedAvg incurs.  

\iffalse

We observe that \textsc{Verdove} achieves a 3$\times$ speedup in the case of 10\% participation and as much as 10$\times$ speedup in the case of 30\%. Moreover, \textsc{VerdoveProx} achieves even further speedups over \textsc{Verdove}, as much as 2$\times$ over the base method. MOON lags in this metric because its additional forward pass calculations incur significant compute penalties. 

The wide gap between FedAvg and FedProx, consistent between 10\% and 30\% cases, suggests the proximal term mitigates client drift without much overhead, as opposed to MOON's contrastive term. \textcolor{red}{Tasos: we talk about a wide gap. Do we assume the reader will understand this gap from the tables? Are we referring to a figure that is missing? Currently, we only have the 30\% cases; would the figure of 10\% cases (side by side) reveal this gap more clearly? One solution to this without including a figure is to use different colors in the table.} 

However, we do not see a similar gap between \textsc{Verdove} and \textsc{VerdoveProx} in the 10\% case but we do in the 30\%. A possible explanation is that in averaged aggregation schemes the proximal term has a greater influence on the local training due to the entire model is being compared against in the proximal term, whereas \textsc{VerdoveProx} isolates the global model's weights by subnetwork.  
\fi

\subsection{Communication Efficiency}

\input{tables/comm_table_10.tex}

\input{tables/comm_table_30.tex}

\input{tables/comm_table_02.tex}

\input{tables/comm_table_06.tex}

\input{tables/comm_table_10_iid.tex}

\begin{figure}
    \centering
    %\input{acc_birds_bytes.tikz}
    \includegraphics[width=0.4\textwidth]{Accuracy over Bytes Transferred (Birds dataset).pdf}
    \caption{\label{fig:birds_bytes} Accuracy over bytes transferred for the CUB-200-2011 dataset in the 30\% case. The dashed line represents the 90\% best accuracy threshold that we compare against. \textcolor{red}{Tasos: same comments as in previous figure.}}
\end{figure}

We use the Python \textit{torchinfo} \cite{torchinfo} package to estimate the number of bytes communicated per synchronization round. As \textsc{Verdove} parititons the global model into disjoint local models, the total bytes communicated to and from the server is size of the model. In contrast, with the averaging algorithms the estimated model size must also be multiplied by the number of participating devices. \cref{table:comm_10}, \cref{table:comm_30}, \cref{table:comm_02}, \cref{table:comm_06}, and \cref{table:comm_10iid} show the number of GB to reach 90\% of the top accuracy for each dataset for respective experimental cases. Again, we have a timeout cutoff, in this case 5000 GB of communication, and mark in the tables "FAIL" in the cases an algorithm does not achieve 90\% accuracy within either this cutoff or the aforementioned one for GFLOP count. 

Again, consistent with our observations with GFLOPs in the i.i.d. case, the communication costs are similar between FedProx and MOON as well as between VERDOVE and VERDOVEProx. Again, VERDOVE methods generally perform best along this metric, except for Stanford Cars and VGG Textures datasets. For the former, FedAvg surprisingly fast convergence with about 5x less communication costs compared the next fastest VERDOVE(PROX). In the latter we note that FedAdam does not have the accuracy gap that it exhibits for some datasets like CUB-Birds or Stanford Cars. However, we noted before that FedAdam reaches rapidly to a peak but then drops off in convergence accuracy. Like the FLOP results, the gap between i.i.d. versus non-i.i.d. exhibits similar tendencies where the former is about 30x faster. However, one interesting exception is FedAvg on the VGGFlowers dataset where the non-i.i.d. 10\% participation case has better communication cost. However, we must be careful when comparing these as the non-i.i.d. case achieves lower final accuracies so these may not be directly comparable. Moreover, we do not see the same behavior in the FLOP results because we find that the optimal local iterations in the non-i.i.d. case uses more local rounds while in the i.i.d. case can suffice with one round per communication phase. 

As with the computation costs, FedAdam and the full ResNet training FedProx methods consistently fail to reach the 90\% threshold within the timeout. However, we note that with the communication costs FedNova is able to achieve similar or better performance than FedAvg in about half the datasets and experiments. This would suggest FedNova in many cases performs more computation per communication round than FedAvg which leads to this disparity. 

In the non-i.i.d. case, VERDOVE methods again generally perform best for all datasets and in most cases, except Stanford Cars and CIFAR100 on communication costs. In the 30\% case we see wide disparities between VERDOVE and VERDOVEProx, although inconsistent on which is better. However in the other scenarios the gap between the two is minor. 
Similarly there is no inherent extra communication overhead for MOON compared to FedProx so we see that their communication costs are around the same and in the cases where there is a wide disparity, e.g. 6\% Stanford Cars or 10\% CIFAR100, there is no clear faster algorithm. 

Unlike with the computation overhead, the communication cost gap between FedAvg and FedProx is narrower and in many cases FedAvg outperforms non-FAIL FedProx, for example 2\% participation Aircraft dataset. This is consistent with our findings in the GFLOP: FedAvg performs more computations per communication round while both methods have roughly the same model communication costs per round. Because FedAvg does more computation per round, it requires fewer total communication rounds and therefore in some cases achieves better communication efficiency.   

Unlike with computation costs, the gigabytes transferred do not show drastic disparities between algorithms. VERDOVE methods do well on the widest range of datasets, but FedAvg, FedProx, and MOON demonstrate good communication costs on multiple datasets and experimental scenarios. 

\iffalse
We observe that in terms of bytes transferred, FedAvg has a slight edge over other averaging algorithms. All of the averaging methods have similar bytes transferred per communication rounds, so this metric favors the method with the fewest communication rounds among them. FedAvg's consistently high FLOP count, as noted in our discussion of compute efficiency, alongside its smaller communication footprint is due to FedAvg performing more local iterations per communication round and trading off more FLOPs for fewer GB transferred. 

Moreover, we see that decomposition methods consistently have better communication performance, especially in the 30\% case, as illustrated in ~\cref{fig:birds_bytes} where we observe that \textsc{Verdove} and \textsc{VerdoveProx} reach the 90\% threshold with fewer bytes transferred. The better communication as client participation increases results from our total communication cost per round being independent of total number of clients. Hence, vertical decomposition scales better with both larger client participation. The extreme case of this is again in the CelebA dataset where \textsc{Verdove} algorithms vastly outperform, by as much as 1000x, over averaging algorithms. 
\fi

\input{tables/acc_table_10.tex}

\input{tables/acc_table_30.tex}

\input{tables/acc_table_02.tex}

\input{tables/acc_table_06.tex}

\input{tables/acc_table_10_iid.tex}

==> intro.tex <==


There has been a lot of recent work aimed at developing and evaluating new algorithms for federated learning, particularly for image classification \cite{}. Most papers in this space are primarily concerned with the development of innovative algorithms, and less concerned with the design of appropriate benchmarks and especially, appropriate baselines to test against. Consider the following concerns regarding the design of the benchmarks and baselines that appear in many federated learning papers.

\vspace{5 pt}
\noindent 
(1) \textit{Learning algorithms are typically evaluated on a few diverse data sets, rather than a large variety of more focused data sets.} The most common benchmark for evaluating federated image classification is CIFAR-100 \cite{}, which includes whales, chairs, dinosaurs, rabbits, and so on. This is a very diverse set of classes, to say the least, and we are concerned that few federated learning tasks will involve differentiating dinosaurs from rabbits.  

For example, imagine that the members of a bird watching club take pictures using their smartphones; club members label the pictures with the bird species, and federated learning is used to build a classifier. Or, a set of companies who are typically competitors—and hence cannot exchange data—want to work together to classify pictures of industrial drill bits based on whether they are going to fail. Both of these deployments involve narrow domains, and the classification problems (classifying birds or  drill bits) involve differentiating among different members of a narrow category. True, not all applications of federated learning will be so narrow, but they are likely to be far narrower than classifying whales versus chairs.  Given this we argue that while evaluating on a broad dataset such as CIFAR-100 is useful, it is also necessary to evaluate federated learning algorithms on a wide variety of more narrow data sets.

\vspace{5 pt}
\noindent 
(2) \textit{Most evaluations focus on final accuracy or the number of communication rounds required for converegence.} In the literature, federated learning algorithms are often evaluated by reporting final accuracies (after convergence), or by plotting test accuracy as a function of the number of epochs, or the number of communication rounds. 

However, final accuracy, at least in isolation, is not really a useful metric. After all, the simplest ``federated learning’’ algorithm is classical, data parallel learning \cite{}. That is, run distributed gradient descent; compute gradients locally over mini-batches in a fully synchronous way, then do an all-reduce \cite{}. As this is functionally equivalent to centralized learning, it is invariant to data distribution, and is likely to be the most accurate method in terms of final accuracy. However, it is inefficient in a federated environment. 

Likewise, considering accuracy as a function of communication rounds ignores the computational or communication cost of each round. Communication and computation costs can vary across methods, and are typically far more important than the number of rounds. A method that can quickly achieve high accuracy with a relatively large number of very inexpensive communication rounds---where a small fraction of the model is communicated at each round---is probably preferred to one that uses few rounds, but must transmit a huge amount of data. 

\vspace{5 pt}
\noindent 
(3) \textit{Pre-trained feature extractors need to be a standard baseline.} Training the feature-extraction backbone that is used in most deep image processing networks--that is, the series of convolutional and pooling layers and without the final classification layer---is not easy, and is perhaps more difficult than actually training the classifier that sits on top of them. It is difficult to get the training process right, and training a good backbone requires a lot of data. 

Researchers have recently suggested using pre-trained backbones, especially for few-shot training \cite{}.  Given the resource constraints in many federated learning scenarios, if is unclear why one would even attempt to train such a backbone in a federated environment, at least as a first approach. Instead, simply take a standard, pre-trained backbone (such the backbone extracted from a ResNet \cite{} or a DenseNet \cite{} or both) and directly use that as a feature extractor. 

The benefit of this approach is that each training image only needs to be pushed through the backbone one time to obtain a compact set of features, and then that set can be used during training. As the backbone need not be communicated or repeatedly used to process the input images, both CPU/GPU cycles and communication is saved during federated training. And furthermore, final accuracies might actually be better, as this approach sidesteps the difficulty of training the backbone. At the very least, this baseline needs to be considered in every study. 

\vspace{5 pt}
\noindent 
\textit (4) \textit{Off-the-shelf performance is really what matters.} In a centralized environment, it is feasible to train and re-train many times, as various parameters  (learning rate, proximal weight, exact neural architecture, etc.) are tuned. In federated learning, this is much less feasible. Again, most federated learning scenarios imagine a resource-contstrained environment (possibly involving edge devices), where one cannot ignore the cost of tuning. Federated learning is typically happening on someone else’s hardware, and so running a learning algorithm many times during parameter tuning is likely to make participation in federated learning far less palatable. 

Furtther, application-specific tuning may simply be impossible. A device may enter the federated training and then drop out shortly after, never to be seen again. One cannot access a missing device’s data to perform validation, and clearly, one cannot retrain over data that cannot be accessed.

As such, we argue that ``off-the-shelf’’ performance is more important than in centralized learning. That is, it becomes important to settle on one set of universal parameters that tend to work will in most or all deployments, so that the learning algorithm can be universally deployed without further tuning. At the very least, this is an important use case that should be covered in most experiments.

\vspace{5 pt}
\noindent
\textbf{A simple method for federated learning over images.} In this paper, we argue for a very simple algorithm for federated image classification, called ``vertical decomposition over a pretrained backbone'' or \textsc{Verdove} for short. \textsc{Verdove}d is designed with the aforementioned considerations in mind. In the paper, we give some strong evidence that this baseline is difficult to beat under realistic scenarios.  

In \textsc{Verdove}, a fully-connected network is decomposed vertically into subnetworks \cite{}, and these vertical subnets are sent to sites for local training. All of this is done over feature vectors extracted using one or more pre-trainted backbones (we advocate using two, quite different backbones, for diversity of features). 

\textsc{Verdove} is especially attractive in the context of the considerations enumerated above.  We find that classical, full backpropogation---where the feature-extraction backbone is trained as well as the classifier---seems to have serious problems with accuracy when trained on a less diverse data set, and a pre-trained backbone works much better.  Further, the pre-trained backbones seem to obviate the need for tuning

Since only narrow subnets are ever communicated to the various sites during federated training of \textsc{Verdove}, communication costs are very low. And because local training happens only over a narrow subnetwork---and the feature extractor is fixed and need only be run one time per image---CPU costs are also very low. 

\vspace{5 pt}
\noindent
\textbf{Our Contributions.}  Our contributions are as follows.

\begin{itemize}
    \item We suggest several rules-of-thumb governing benchmark and baseline development for federated learning over images, and use those rules to devise an extensive federated image classification benchmark, and use that benchmark to carefully evaluate a number of options for federated learning over images.

    \item We use those rules to devise a very simple federated learning algorithm---\textsc{Verdove}---which by design does well in a resource constrained environment where CPU cycles and communication are precious and the classification task is difficult, in the sense that involves differentiating between similar objects.

    \item Our benchmark shows that \textsc{Verdove} may be quite difficult to beat, even for state-of-the-art methods.  

    \item We do some additional experiments that attempt to explain why the vertical decompositions or ``subnets'' used by \textsc{Verdove} are particularly useful for federated learning over data that are skewed, in the sense that only a few classes reside at each site.
\end{itemize}





==> tables/diric_skew_birds.tex <==
\begin{table*}[!hb]
\caption{Average number of classes per user on different Dirichlet concentration $\alpha$ on CUB-200-2011}
\centering
\begin{tabular}{cccccccc}
\hline
        $\alpha$ &  Average number of classes (\% of total classes) \\ 
       \hline
100  & 199.83 (99.92\%)  \\
    \hline
10 & 199.72 (99.86\%) \\
    \hline
1  & 163.97 (81.99\%) \\
    \hline
0.1  & 59.73 (29.87\%) \\
    \hline
0.01 & 11.77 (5.89\%)  
\end{tabular}
\label{table:diric_skew_birds}
\vspace{-0.3cm}
\end{table*}

==> tables/method_comparison.tex <==
\begin{tabular}{cccccccc}
\multicolumn{7}{c}{Comparison of different federated learning algorithms} \\
\hline
Alg & Type & Proximal & Time Comp.\\ 
\hline
    FedAvg & Avg & No & $O(mnt)$\\
    FedProx & Avg & Yes & $O(mnt)$\\
    MOON & Avg & Yes & $O(mnt)$\\
    FedAdam & Avg & No & $O(mnt)$\\
    FedNova & Avg & No & $O(mnt)$\\
    IST & Decomp & No & $O(mt)$\\
    ISTProx & Decomp & Yes & $O(mt)$\\
\hline
\end{tabular}
\label{table:method_compare}
